Training Stable Graph Neural Networks Through Constrained Learning

Graph Neural Networks (GNN) rely on graph convolutions to learn features from network data. GNNs are stable to different types of perturbations of the underlying graph, a property that they inherit from graph filters. In this paper we leverage the stability property of GNNs as a typing point in order to seek for representations that are stable within a distribution. We propose a novel constrained learning approach by imposing a constraint on the stability condition of the GNN within a perturbation of choice. We showcase our framework in real world data, corroborating that we are able to obtain more stable representations while not compromising the overall accuracy of the predictor.

==> latex_resources/my_sections.tex <==
\usepackage{needspace}

% \nbsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsection}[1]{\needspace{1\baselineskip}\color{white}\medskip\subsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsection\quad #1.}}



% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}
